Detecting individual-level infections using sparse group-testing through graph-coupled hidden Markov models

Identifying the infection status of each individual during infectious diseases informs public health management. However, performing frequent individual-level tests may not be feasible. Instead, sparse and sometimes group-level tests are performed. Determining the infection status of individuals using sparse group-level tests remains an open problem. We have tackled this problem by extending graph-coupled hidden Markov models with individuals infection statuses as the hidden states and the group test results as the observations. We fitted the model to simulation datasets using the Gibbs sampling method. The model performed about 0.55 AUC for low testing frequencies and increased to 0.80 AUC in the case where the groups were tested every day. The model was separately tested on a daily basis case to predict the statuses over time and after 15 days of the beginning of the spread, which resulted in 0.98 AUC at day 16 and remained above 0.80 AUC until day 128. Therefore, although dealing with sparse tests remains unsolved, the results open the possibility of using initial group screenings during pandemics to accurately estimate individuals infection statuses.

==> notes.tex <==
1) Make sure to say that our algorithm is inpsired by ....

==> settings.tex <==
%!TEX encoding = UTF-8 Unicode
% packages and settings for BeLLS
% all packages are available in standard LaTeX distributions such as MacTeX 2016

% page layout (text area is 126mm, 196mm)
\usepackage[papersize={17cm,24cm},margin=22mm,top=17mm,headsep=5mm]{geometry} 

\usepackage{xltxtra} % extras for XeLaTeX
\usepackage{verbatim} % verbatim input
\usepackage{titling} % customize title
\usepackage{csquotes} % context sensitive quotes
\usepackage{upquote} % allow correct quotes in verbatim
\usepackage[bottom]{footmisc} % put footnotes down at the bottom margin
\usepackage[svgnames]{xcolor} % color pictures with SVG names
\usepackage{graphicx} % \includegraphics
\usepackage{enumitem} % customize lists
%\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
\setitemize{itemsep=2pt,topsep=4pt,parsep=0pt,partopsep=0pt}
\usepackage{covington}  % for numbered linguistic examples

%\usepackage[english]{babel} % multilinguality
\usepackage{polyglossia} % newer alternative to babel
\setdefaultlanguage{english} % see http://ctan.uib.no/macros/xetex/latex/polyglossia/polyglossia.pdf

\setmainfont[Mapping=tex-text,Ligatures=TeX,Scale=1.0]{Linux Libertine O} 
\setmonofont[Mapping=tex-text,Scale=MatchLowercase,LetterSpace=-2.0]{DejaVu Sans Mono}
\renewcommand{\baselinestretch}{1.04} % stretch distance between baselines
\frenchspacing % reduce space after sentence-final punctuation
\date{}
\setlength{\parindent}{1em}
\clubpenalty = 10000
\widowpenalty = 10000
\hfuzz = 2pt  % No warnings about margin overhangs less than this amount.
%\setlength{\belowcaptionskip}{-1.2em}

\usepackage[backend=biber, style=authoryear, citestyle=authoryear-comp, maxcitenames=2, maxbibnames=50, language=auto, isbn=false, url=false]{biblatex} % new alternative to bibtex
\setlength{\bibhang}{\parindent}
\usepackage[breaklinks,colorlinks,urlcolor=black,citecolor=black,linkcolor=black]{hyperref} % pagebackref incompatible with biblatex

\usepackage[compact,noindentafter]{titlesec} % customize section headings
\titlespacing{\section}{0pt}{2.7mm}{1.5mm} % left indent, space before, space after
\titlespacing{\subsection}{0pt}{2mm}{1pt}
\titlespacing{\subsubsection}{0pt}{1.2mm}{0.5pt}

\newcommand\Volume{N} % BeLLS Volume number
\newcommand\Voleditors{Jan Editor and Ed Janitor}
\newcommand\Voltitle{The book title}
\newcommand\VolISBN{N}
\newcommand\VolDOI{N}

%\usepackage{natbib}
%\usepackage{fullname}
%\bibliographystyle{fullname} % chicago or spbasic or spmpsci or spphys
%\setlength{\bibhang}{-0.5em}
%\setlength{\bibsep}{0mm}
%\let\bibfont=\small

% footnote without number
\newcommand\blfootnote[1]{
  \begingroup
  \renewcommand\thefootnote{}\footnote{\hspace{-2.4em} #1}%
  \addtocounter{footnote}{-1}
  \endgroup
}

% customize title
\renewcommand{\maketitle}
  {\bgroup\setlength{\parindent}{0pt}
   \begin{flushleft}
    \textbf{\LARGE{\ \\ \vspace{20mm}\strut\thetitle\strut}\vspace{2mm}}
    
    {\Large\theauthor}
  \end{flushleft}\egroup\vspace{18mm}
}

% customize abstract
\renewenvironment{abstract}
  {\noindent\small %\quotation
  {\noindent{\large\textbf\abstractname. }%\par\nobreak\smallskip
  \thispagestyle{plain}
  %\blfootnote{In: \emph{Volume title,} edited by Jan Editor and Ed Janitor. BeLLS Vol. N (2017), DOI N. Open Access under the terms of CC-BY-NC-4.0.}
  }}
  {}
    
% command in which to embed tabular material in numbered example
% use: \begin{example}\extab\begin{tabular ...
\newcommand{\extab}[2][-0.69\baselineskip]{ 
   \parbox[t]{.9\textwidth}{
     \setlength{\tabcolsep}{1.3pt} % use small space between columns
     \vspace{#1}
     #2
    }
}

% command to put ref in parentheses
\newcommand{\refp}[1]{(\ref{#1})}

% customize page headers
\usepackage{fancyhdr}
\pagestyle{fancy}
\renewcommand{\headrulewidth}{0.4pt}
\fancyhead{}  \fancyfoot{} %clear
\makeatletter % necessary for commands with @
  \fancyhead[RO]{\small\textit{\@title}}
  \fancyhead[LE]{\small\textit{\@author}}
\makeatother
%\fancyhead[RE]{\small BeLLS Vol. \Volume}
 % no footer
\setlength{\headheight}{20.68pt} % room for two lines
\fancypagestyle{plain}{% first page of chapter
 %\fancyhead[L]{}
 \fancyhead[L]{\footnotesize In: \emph{Volume title,} edited by Jan Editor and Ed Janitor. BeLLS Vol. N (2017), DOI N. Open Access under the terms of CC-BY-NC-4.0.} % comment to keep the normal header
  \fancyhead[C,R]{}
  %\renewcommand{\headrulewidth}{0pt} % comment to keep rule
  \fancyfoot{} % comment to put page number at bottom
  }



